Dependency-Aware Rollback and Checkpoint-Restart for Distributed Task-Based Runtimes

With the increase in compute nodes in large compute platforms, a proportional increase in node failures will follow. Many application-based checkpoint/restart (C/R) techniques have been proposed for MPI applications to target the reduced mean time between failures. However, rollback as part of the recovery remains a dominant cost even in highly optimised MPI applications employing C/R techniques. Continuing execution past a checkpoint (that is, reducing rollback) is possible in message-passing runtimes, but extremely complex to design and implement. Our work focuses on task-based runtimes, where task dependencies are explicit and message passing is implicit. We see an opportunity for reducing rollback for such runtimes: we explore task dependencies in the rollback, which we call dependency-aware rollback. We also design a new C/R technique, which is influenced by recursive decomposition of tasks, and combine it with dependency-aware rollback. We expect the dependency-aware rollback to cancel and recompute less tasks in the presence of node failures. We describe, implement and validate the proposed protocol in a simulator, which confirms these expectations. In addition, we consistently observe faster overall execution time for dependency-aware rollback in the presence of faults, despite the fact that reduced task cancellation does not guarantee reduced overall execution time.

==> checkpoints.tex <==
\begin{figure}[t]
\centering
    \begin{tikzpicture} []
        \draw (0,0) -- (3,0) -- (3,3) -- (0,3) -- (0,0) -- (3,3);
        \draw (3,0) -- (0,3);
		\draw (0,1.5) -- (3,1.5) -- (1.5,0) -- (0,1.5) -- (1.5,3) -- (3,1.5);
		\draw (0.75,0.75) -- (2.25,0.75);
		\draw (0.75,2.25) -- (2.25,2.25);
		\draw[red] (0,0) -- (0.75,0.75) -- (1.5,0) -- (2.25,0.75) -- (3,0);
       \node (a) [] at (0.75,0.25) {1};
        \node (b) [] at (1.5,0.45) {3};
        \node (c) [] at (2.25,0.25) {2};
	\begin{scope}[{xshift=4cm}]    
        \draw (0,0) -- (3,0) -- (3,3) -- (0,3) -- (0,0) -- (3,3);
        \draw (3,0) -- (0,3);
        \draw[red] (3,0) -- (0,3);
		\draw (0,1.5) -- (3,1.5) -- (1.5,0) -- (0,1.5) -- (1.5,3) -- (3,1.5);
		\draw (0.75,0.75) -- (2.25,0.75);
		\draw (0.75,2.25) -- (2.25,2.25);        
   

        \node (a) [] at (2.25,0.25) {1};
        \node (b) [] at (1.5,0.45) {2};
        \node (c) [] at (1.5,1.15) {3};
        \node (d) [] at (0.75,1.25) {4};
        \node (e) [] at (0.75,1.95) {5};
        \node (f) [] at (0.25,2.05) {6};
        
        \end{scope}

    \end{tikzpicture}

    \caption{Two different possible processing orders: one horizontal, and one diagonal. This has implications to the checkpointing, which may scale better with more parallelism (left) rather than with more sequentiality (right).}
    \label{fig:checkpoints}
\end{figure}


==> consistent-cps.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[scale=1.5]

\node (a) at (0,0){}; 
\node (b) at (3,0) {};
\node (c) at (4.5,3) {};
\node (d) at (1.5,3) {};
\node (ab) at ($(a)!0.5!(b)$) {};
\node (ab2) at ($(a)!0.25!(b)$) {};
\node (ab3) at ($(a)!0.75!(b)$) {};
\node (cd) at ($(c)!0.5!(d)$) {};
\node (cd2) at ($(c)!0.25!(d)$) {};
\node (cd3) at ($(c)!0.75!(d)$) {};
\node (bc) at ($(b)!0.5!(c)$) {};
\node (bc2) at ($(b)!0.25!(c)$) {};
\node (bc3) at ($(b)!0.75!(c)$) {};
\node (ad) at ($(a)!0.5!(d)$) {};
\node (ad2) at ($(a)!0.25!(d)$) {};
\node (ad3) at ($(a)!0.75!(d)$) {};
\node (mid) at ($(a)!0.5!(c)$) {};
\path[draw]  (a) -- (b) -- (c) -- (d) -- (a);
\path[draw] (ad) -- (ab) -- (cd) -- (bc) -- (ad);
\path[draw] (b) -- (d);
\path[draw] (ad2) -- (bc2);
\path[draw] (ad3) -- (bc3);
\path[draw] (ab3) -- (cd2);
\path[draw] (ab2) -- (cd3);
\path[draw] (ab3) -- (ad3);
\path[draw] (bc2) -- (cd3);
\path[draw] (ab2) -- (ad2);
\path[draw] (bc3) -- (cd2);
\begin{scope}[on background layer]
	\draw [fill=red] (1.5,1.5) -- (2.25,1.5) -- ($(3.75/2,2.25)$) ;
	\draw [fill=yellow!80!red] (1.5,1.5) -- (2.25,1.5) -- ($(5.25/2,0.75)$) -- ($(2.25/2,0.75)$) ;
	\draw[fill=yellow!40] ($(2.25/2,0.75)$) -- (0.75,1.5) -- ($(2.25/2,2.25)$) -- (1.5,1.5);
	\draw[fill=yellow!40] ($(5.25/2,0.75)$) -- (2.25,1.5) -- ($(5.25/2,2.25)$) -- (3.,1.5);
	\draw[fill=green!40] (0.75,1.5) -- (0,0) -- (3,0) -- ($(8.25/2,2.25)$) --  ($(6.75/2,2.25)$) -- ($(5.25/2,0.75)$) -- ($(2.25/2,0.75)$);
\end{scope}
\draw[blue,ultra thick] ($(2.25/2,0.75)$) --  ($(5.25/2,0.75)$) -- ($(3.75/2,2.25)$) -- ($(2.25/2,0.75)$);
\node[] at (current bounding box.west) {
\begin{tabular}{@{}r@{ }l@{}}
 \raisebox{2pt}{\tikz{\draw [fill=red] (0,0) -- (0.5,0) -- (0.25,0.5);}}&failed\\
 \raisebox{2pt}{\tikz{\draw [fill=yellow!80!red] (0,0) -- (0.5,0) -- (0.25,0.5);}}&checkpointed\\
 \raisebox{2pt}{\tikz{\draw [fill=yellow!40] (0,0) -- (0.5,0) -- (0.25,0.5);}}&cancelled \\
  \raisebox{2pt}{\tikz{\draw [fill=green!40] (0,0) -- (0.5,0) -- (0.25,0.5);}}&fine
\end{tabular}};
\end{tikzpicture}
\caption{Minimal rollback of tasks when a worker fails: Tasks marked in orange are cancelled since their checkpoints can reproduce the failed task. Tasks in yellow are cancelled since they depend on orange tasks. No tasks in green need to be cancelled.}
\label{fig:consistent-cps}
\end{figure}
